Arena-Rosnav: Towards Deployment of Deep-Reinforcement-Learning-Based Obstacle Avoidance into Conventional Autonomous Navigation Systems

Recently, mobile robots have become important tools in various industries, especially in logistics. Deep reinforcement learning emerged as an alternative planning method to replace overly conservative approaches and promises more efficient and flexible navigation. However, deep reinforcement learning approaches are not suitable for long-range navigation due to their proneness to local minima and lack of long term memory, which hinders its widespread integration into industrial applications of mobile robotics. In this paper, we propose a navigation system incorporating deep-reinforcement-learning-based local planners into conventional navigation stacks for long-range navigation. Therefore, a framework for training and testing the deep reinforcement learning algorithms along with classic approaches is presented. We evaluated our deep-reinforcement-learning-enhanced navigation system against various conventional planners and found that our system outperforms them in terms of safety, efficiency and robustness.

==> ieeeconf/content/acknowledgment.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex



==> ieeeconf/content/keywords.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex


%\begin{IEEEkeywords}
%	Virtual Reality and Interfaces, Localization, Object Detection, Computer Vision for Other %Robotic Applications, AI-Based Methods
%\end{IEEEkeywords}

==> ieeeconf/content/title.tex <==
% !TeX encoding = utf-8
% !TeX language = en_GB
% !TeX spellcheck = en_GB
% !TeX root = paper.tex

%\title{A robust pose estimator for articualted robots using monocular cameras and Deep-Learning-based keypoint detection\\
%	}
%	\thanks{Identify applicable funding agency here. If none, delete this.}
%}
\title{\LARGE \bf
Towards Augmented Reality Simulation in Robotics - Facing Barriers of Industrial Applicability
}

\author{Jens Lambrecht$^{1}$, Linh Kästner$^{1}$, Jan Guhl$^{2}$ and J\"org Kr\"uger$^{2}$% <-this % stops a space% <-this % stops a space
% \thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Jens Lambrecht and Linh Kästner are with the Chair Industry Grade Networks and Clouds, Faculty of Electrical Engineering and Computer Science,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small lambrecht@tu-berlin.de}}%
\thanks{$^{2}$Jan Guhl and J\"org Kr\"uger are with the Chair Industrial Automation Technology, Faculty of Mechanical Engineering and Transport Systems,
        Technische Universität Berlin, 10587 Berlin, Germany
        {\tt\small guhl@iat.tu-berlin.de}}%        
}


%\author{
%	\IEEEauthorblockN{Jens Lambrecht}
%	\IEEEauthorblockA{\textit{Chair Industry Grade Networks and Clouds} \\
%		\textit{Technische Universität Berlin}\\
%		Berlin, Germany \\
%		lambrecht@tu-berlin.de}
%}

\maketitle
